Sequenced Route Query with Semantic Hierarchy

The trip planning query searches for preferred routes starting from a given point through multiple Point-of-Interests (PoI) that match user requirements. Although previous studies have investigated trip planning queries, they lack flexibility for finding routes because all of them output routes that strictly match user requirements. We study trip planning queries that output multiple routes in a flexible manner. We propose a new type of query called skyline sequenced route (SkySR) query, which searches for all preferred sequenced routes to users by extending the shortest route search with the semantic similarity of PoIs in the route. Flexibility is achieved by the {\it semantic hierarchy} of the PoI category. We propose an efficient algorithm for the SkySR query, bulk SkySR algorithm that simultaneously searches for sequenced routes and prunes unnecessary routes effectively. Experimental evaluations show that the proposed approach significantly outperforms the existing approaches in terms of response time (up to four orders of magnitude). Moreover, we develop a prototype service that uses the SkySR query, and conduct a user test to evaluate its usefulness.

==> algorithms/OSRbased.tex <==
\begin{algorithm}[h]
	\caption{OSR-based solution that repeats OSR query algorithm until all skyline sequenced routes have been found}	\label{alg:osr-based}
	       
	            \SetKwFunction{OSR}{OSR}
	            {\bf procedure} Naive algorithm($q$, $S_q$)\\
	            \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	            %\Input{start point $q$, category sequence $M_q$}
	           % \Output{$\mathcal{SKY}$}
		              $\mathcal{SKY}$ $\leftarrow$ $\phi$;\\
		               $\mathcal{SUP} (S_q) \leftarrow$  super-category sequences of $S_q$;\\
                       \For{$\forall S \in \mathcal{SUP} (S_q)$}{
		                      $SR_{osr}$ $\leftarrow$ \OSR{\textit{$q$, $S$}};\\
		                      $\mathcal{SKY}$.update($SR_{osr}$);
                        }       
                        return $\mathcal{SKY}$;\\
              {\bf end procedure}\\
                
\end{algorithm}


==> algorithms/improvedOSR.tex <==
\begin{algorithm}[h]
	\caption{OSR-based algorithm using the upperbound}	\label{alg:imp-osr}
	            \SetKwFunction{OSR}{mOSR}
	             \SetKwFunction{NNbasedEst}{NNmethod}
	              \SetKwFunction{UOSR}{UOSR}
	              \SetKwFunction{upperbound}{ub}
	            \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	            {\bf procedure} \UOSR{$q$,$S_q$}\\
		                 $\mathcal{SUP} (S_q) \leftarrow$  super-category sequences of $S_q$;\\
		                sort $\mathcal{SUP} (S_q) $ in ascending order of $dssim(S_q, S_{q_{sup}})$;\\		              
		                $\mathcal{SKY} \leftarrow$ \NNbasedEst{\textit{$q$, $S_q$}};\\
		                $ub \leftarrow$ \upperbound{${\mathrm 0}$};\\
                       \For{$\forall S \in \mathcal{SUP} (S_q)$}{
		                      $ub \leftarrow$ \upperbound{$dssim(S_q,S)$};\\
		                      $SR_{osr}$ $\leftarrow$ \OSR{\textit{q, $S$, ub}};\\
		                      $\mathcal{SKY}$.update($SR_{osr}$);
                        }
               return $\mathcal{SKY}$;\\
               {\bf end procedure}
\end{algorithm}


==> algorithms/partialUB.tex <==
\begin{algorithm}[h]
	\caption{Partial upperbound calculation}	\label{alg:ub_p}
		\DontPrintSemicolon
			    \SetKwFunction{MinUB}{MinUB}
			    \SetKwFunction{nextPoI}{nextPoI}
			      \SetKwFunction{NNbasedEst}{NNbasedEstimation}
	            \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	            \Input{route \textit{R}, NN-based length $l_{NN}$}
		       $ub_p \leftarrow  (R.n + 1)\cdot \frac{\texttt{ub}(ds(R))}{m}$;\\     
		       \lIf{ $ub_p$ $<$ $l_{NN}[R.n] $}{$ub_p \leftarrow l_{NN}[R.n] $;}
\end{algorithm}

